Accelerated Multiplicative Weights Update Avoids Saddle Points almost always

We consider non-convex optimization problems with constraint that is a product of simplices. A commonly used algorithm in solving this type of problem is the Multiplicative Weights Update (MWU), an algorithm that is widely used in game theory, machine learning and multi-agent systems. Despite it has been known that MWU avoids saddle points, there is a question that remains unaddressed:"Is there an accelerated version of MWU that avoids saddle points provably?" In this paper we provide a positive answer to above question. We provide an accelerated MWU based on Riemannian Accelerated Gradient Descent, and prove that the Riemannian Accelerated Gradient Descent, thus the accelerated MWU, almost always avoid saddle points.

==> experiment.tex <==
\newpage

\section{Experiments}
In this section we present three kinds of numerical experiments of our results, they are:
\begin{itemize}
\item[(1)]  Trajectories of accelerated MWU algorithm with test function $f_1$ and $f_2$ (figure \ref{img 2}). Since the domain is $\Delta^{2}_+$, $f_1,f_2$ are equivalent to  $\tilde{f_1 }(x,y) = \cos(8.5x) \sin(8.5(y-0.4)) + \sin(8.5(1-x-y))$ and $\tilde{f_2}(x,y) = 0.5\cos(5(x-0.31)) \sin(5(y-0.32)) \sin(5(1-x-y))$, the backgrounds are contour lines of  $\tilde{f_1 }$ and $\tilde{f_2 }$.
\item[(2)]  Convergence curves of accelerated MWU and non- accelerated case for some $g :\Delta^{2}_+ \to \mathbb{R}$ (figure \ref{img 3}) .
\item[(3)]  Convergence curves of accelerated MWU and non- accelerated case for some $h :\Delta^{1}_+ \times \Delta^{1}_+ \to \mathbb{R}$ (figure \ref{img 4}).
\end{itemize}

In figure \ref{img 2}, note that both of these two graphs have a saddle point near the initial values, and trajectories not fall into these saddle points, this support one of the main results in this paper : Accelerated MWU always avoids saddle points. 

In figure \ref{img 3} and figure \ref{img 4}, both of these two cases accelerated method converges faster than ordinary method, especially in the first picture of  figure \ref{img 3}, the trajectories meet a saddle point, and we can clearly see accelerated method escapes faster than ordinary method, which support our theoretical analysis for the non-asymptotic convergence rate and efficiency in escaping saddle points of accelerated method. 




\begin{figure} [H]
	\centering
	\begin{minipage}[c]{0.5\textwidth}
	\centering
	 \includegraphics[width=1.6in]{planegraph_1.jpg}
	\end{minipage}% 
	\begin{minipage}[c]{0.5\textwidth}
	\centering \includegraphics[width=1.6in]{planegraph_2.jpg} 
	\end{minipage}
	\caption{$f_1 (x,y,z) = \cos(8.5x) \sin(8.5(y-0.4)) + \sin(8.5z)$ (left) , $f_2(x,y,z) = 0.5\cos(5(x-0.31)) \sin(5(y-0.32)) \sin(5z)$ (right) with initial points $(0.42,0.25,0.33), (0.35,0.5,0.15)$, red = low function values.  } 
	\label{img 2}
\end{figure}


\begin{figure} [H]
	\begin{minipage}[c]{0.5\textwidth}
	\centering \includegraphics[width=1.6in]{linegraph_1_initial_value(0.6,0.2,0.2).png}
	\end{minipage}% 
	\begin{minipage}[c]{0.5\textwidth}
	\centering \includegraphics[width=1.6in]{linegraph_1_initial_value(0.1,0.4,0.5).png} 
	\end{minipage}
	\centering
	\caption{$g(x,y,z) =\cos(0.7x) \sin(y) \sin(0.9z)+x^2$, with initial values$(0.6,0.2,0.2)$ (left) and $(0.1,0.4,0.5)$ (right).} 
	\label{img 3}
\end{figure}




\begin{figure} [H]
	\centering
	\begin{minipage}[c]{0.5\textwidth}
	\centering \includegraphics[width=1.6in]{twosimplice_1_initial_value(0.6,0.4,0.6,0.4).png}
	\end{minipage}% 
	\begin{minipage}[c]{0.5\textwidth}
	\centering \includegraphics[width=1.6in]{twosimplice_1_initial_value(0.7,0.3,0.3,0.7).png} 
	\end{minipage}
	\caption{$h(x,y,z,w) = x^2\sin(y) + z^3\cos(w)$, with initial values $(0.6,0.4,0.6,0.4)$(left) and $(0.7,0.3,0.3,0.7)$ (right).} 
	\label{img 4}
\end{figure}



